Compositionality and Generalization in Emergent Languages

Natural language allows us to refer to novel composite concepts by combining expressions denoting their parts according to systematic rules, a property known as \emph{compositionality}. In this paper, we study whether the language emerging in deep multi-agent simulations possesses a similar ability to refer to novel primitive combinations, and whether it accomplishes this feat by strategies akin to human-language compositionality. Equipped with new ways to measure compositionality in emergent languages inspired by disentanglement in representation learning, we establish three main results. First, given sufficiently large input spaces, the emergent language will naturally develop the ability to refer to novel composite concepts. Second, there is no correlation between the degree of compositionality of an emergent language and its ability to generalize. Third, while compositionality is not necessary for generalization, it provides an advantage in terms of language transmission: The more compositional a language is, the more easily it will be picked up by new learners, even when the latter differ in architecture from the original agents. We conclude that compositionality does not arise from simple generalization pressure, but if an emergent language does chance upon it, it will be more likely to survive and thrive.

==> relatedWork.tex <==
\section{Related Work}

\iffalse
Several works have studied the emergence of language and how it relates to natural language properties \cite{Havrylov:Titov:2017, Chaabouni:etal:2019, kharitonov2019information}. In this context, one of the most studied natural property is \emph{compositionality} \cite{mordatch2018emergence, Steels:2003, nowak2000evolution, kirby1999syntax, cogswell2019} as it is considered to derive productivity (i.e. refering to an infinite number of concepts) \cite{Lazaridou:etal:2018}.
%The study of how compositional structure emerged in natural languages or how it can be enforced in the emergent ones has seen a lot of interest by different communities \cite{mordatch2018emergence, Havrylov:Titov:2017, Steels:2003, nowak2000evolution, kirby1999syntax, cogswell2019}. This research line has long been motivated by the belief that compositionality is the origin of language productivity, one of the most important and practical natural language properties \cite{Lazaridou:etal:2018}.\\
We revise this claim by studying the relation between compostionality and productivity of deep-agent emergent languages. Having deep-agents playing a reconstruction game, we first demonstrate, contrary to previous claim \cite{Kottur:etal:2017}, their ability to develop productive languages if trained on large input samples. This relates to \citet{zhao2018} that investigates generative model generalization w.r.t different training distribution. However the goal of their work is to examine the generative model's inductive bias, whereas we focus on the importance of analyzing emergent languages in rich environment to witness the emergence of interesting properties. Second, we experimentally show that compositionality is not necessary for productivity and hence the latter should not be considered as a proxy for studying the compositional structure of the language. Finally, we show that the degree of language compositionality correlates with the ease of acquisition and use of that language by new learners. The observation persists even when introducing an adversarial loss that enforces certain type of compostionality. These results suggest that transmission ease and efficiency to new learners could be the responsible of the compositional structure of natural language. This is in line with \citet{Li2019} experiments that show that introducing a transmission ease loss do encourage the emergence of compositional structure.
%\cite{Li2019}: the goal of their work is to enforce the emergence of compostitional language with a specific environmental pressure. But they also demonstrated using hand-crafted languages that compositional languages are easier to acquire. We focus instead on only emergent languages with a large spread of degree of compositionality.\\
%\cite{Lake:Baroni:2017, Kottur:etal:2017} suggest that neural networks fails to generalize because of their failure to discover compositional structure. We hypothesise that this is the case because of their limited small training set.\\
%Compositionality vs ease of learning \cite{Li2019}: the goal of their work is to enforce the emergence of compostitional language with a specific environmental pressure. But they also demonstrated using hand-crafted languages that compositional languages are easier to acquire. We focus instead on only emergent languages with a large spread of degree of compositionality.\\
%Generalization vs training distribution \cite{zhao2018}: study generative model generalization w.r.t different training distribution to investigate the model bias. We aim only demonstrate that generalization is possible for large training samples and do not claim anything about the impact on model's inductive bias.\\
\fi
In the context of representation learning, there is a focus towards learning a \emph{disentangled} representation where the independent factors of variation of the data are encoded into independent axes of the latent code. Indeed, by capturing the underlying data structure, such a representation is expected to enable a consequent model (e.g. a classifier) to generalize on new domains and tasks \citep{Bengio2013}. Different models and metrics have been proposed to achieve disentanglement, see \citet{Suter2019} for a review. While there is little consensus on the exact definition of disentanglement as noted in \citet{Higgins2018}, existing works agree on the importance of the \emph{modularity} property: Each dimension of the representation participates in encoding of no more than a single factor of variation of the data. In language, a message can be viewed as a discrete representation carrying information about an object, and generalization would mean successful communication between two agents talking about that object. Therefore, we develop our posdis metric (described in Section ADD) as a metric of linguistic compositionality, taking inspiration from the FactorVAE disentanglement metric \cite{Kim2018} such that each position in the message should correspond to a unique semantical aspect of the input (e.g. its color). Note that existing works challenge the relationship between disentanglement and generalization \citep{Bozkurt2019, Locatello2019}. Similarly, in this paper we question the connection between linguistic compositionality and generalization abilities. We differ from these works as we consider recurrent architectures, and measure linguistic compositionality with our posdis metric, but also existing metrics typically employed in the emergent communication literature (e.g. topographic similarity).

